Compact Symmetric Objects -- I Towards a Comprehensive Bona Fide Catalog

Compact Symmetric Objects (CSOs) are jetted Active Galactic Nuclei (AGN) with overall projected size <1 kpc. The classification was introduced to distinguish these objects from the majority of compact jetted-AGN in centimeter wavelength very long baseline interferometry observations, where the observed emission is relativistically boosted towards the observer. The original classification criteria for CSOs were: (i) evidence of emission on both sides of the center of activity, and (ii) overall size <1 kpc. However some relativistically boosted objects with jet axes close to the line of sight appear symmetric and have been mis-classified as CSOs, thereby undermining the CSO classification. This is because two essential CSO properties, pointed out in the original papers, have been neglected: (iii) low variability, and (iv) low apparent speeds along the jets. As a first step towards creating a comprehensive catalog of ``bona fide'' CSOs, we identify 79 bona fide CSOs, including 15 objects claimed as confirmed CSOs here for the first time, that match the CSO selection criteria. This sample of bona fide CSOs can be used for astrophysical studies of CSOs without contamination by mis-classified CSOs. We show that the fraction of CSOs in complete flux density limited AGN samples with S$_{\rm 5\,GHz}$ >700 mJy is between $(6.8\pm1.6)$% and $(8.5\pm1.8)$%.

==> macros.tex <==
% MACROS.TEX contains generally useful macros, but not those specifically 
%            useful for paper formats.
%
\newcount\figureno  \newcount\tableno
\figureno=0         \tableno=0
%
\newbox\tablebox    \newdimen\tablewidth
%
\newbox\marginbox
\def\strutdepth{\dp\strutbox}
\def\strutheight{\ht\strutbox}
%
\def\smallformat{\hsize=5.5truein\hoffset=0.5truein
    \vsize=8truein\voffset=0.5truein\parskip=1pt}
\def\largeformat{\hsize=6.5truein\hoffset=0.0truein
    \vsize=8.5truein\voffset=0.0truein}
%
\newcount\sectionnumber \newcount\subsectionnumber 
\newcount\subsubsectionnumber
\sectionnumber=0 \subsectionnumber=0 \subsubsectionnumber=0
%
\def\secno{\ifcase\sectionnumber\or
     I\or II\or III\or IV\or V\or VI\or VII\or VIII\or IX\or
     X\or XI\or XII\fi}
\def\subsecno{\ifcase\subsectionnumber\or
     a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\fi}
\def\subsubsecno{\ifcase\subsubsectionnumber\or
     i\or ii\or iii\or iv\or v\or vi\or vii\or viii\or ix\or x\fi}
%
\def\section#1\par{\advance\sectionnumber by 1 \subsectionnumber=0
    \vskip 14pt plus 3pt minus 3pt\goodbreak
    \centerline{{\sc\secno.\ #1}}\nobreak\medskip}
\def\subsection#1\par{\advance\subsectionnumber by 1 \subsubsectionnumber=0
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\it\subsecno\/})\ {\it #1}}\nobreak\medskip}
\def\subsubsection#1\par{\advance\subsubsectionnumber by 1
    \ifdim\lastskip=\medskipamount\nobreak\vskip 8.5pt plus 2pt minus 2pt
       \else \vskip 8.5pt plus 2pt minus 2pt\goodbreak\fi
    \centerline{{\eightrm\subsubsecno)}\ {\it #1}}\nobreak\medskip}
%
\def\today{\ifcase\month\or
    January\or February\or March\or April\or May\or June\or
    July\or August\or September\or October\or November\or December\fi
    \space\number\day, \number\year}
%
\def\sol{\ifmmode _{\mathord\odot}
         \else $_{\mathord\odot}$\fi}
\def\deg{\ifmmode ^{\circ}
         \else $^{\circ}$\fi}
\def\pdeg{\ifmmode $\setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}
          \else \setbox0=\hbox{$^{\circ}$}\rlap{\hskip.11\wd0 .}$^{\circ}$\fi}
% Tony's definitions
\def\vs6{{\vskip 6pt \noindent}}
\def\vs15{{\vskip 15pt \noindent}}
%
\def\arcs{\ifmmode {^{\scriptscriptstyle\prime\prime}}
          \else $^{\scriptscriptstyle\prime\prime}$\fi}
\def\arcm{\ifmmode {^{\scriptscriptstyle\prime}}
          \else $^{\scriptscriptstyle\prime}$\fi}
\newdimen\sa  \newdimen\sb
\def\parcs{\sa=.07em \sb=.03em
     \ifmmode $\rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa$
     \else \rlap{.}$^{\scriptscriptstyle\prime\kern -\sb\prime}$\kern -\sa\fi}
\def\parcm{\sa=.08em \sb=.03em
     \ifmmode $\rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb$
     \else \rlap{.}\kern\sa$^{\scriptscriptstyle\prime}$\kern-\sb\fi}
%
\def\s#1{{\sc #1}}
\def\et{\hbox{\it et al.}}
\def\ET{{\it ET AL.}}
\def\expo#1{\ifmmode \times 10^{#1}
            \else $\times 10^{#1}$\fi}
\def\page{\vfill\eject}
\def\leaderfil{\leaders\hbox to 5pt{\hss.\hss}\hfil}
%
\def\mo{\ifmmode ^{-1}
        \else $^{-1}$\fi}
\def\sup#1{$^{\rm #1}$}
\def\mag{\sup{m}}
\def\muK{\,$\mu$\hbox{K}}
\def\,{\thinspace}
\def\tc#1{3C\,#1}
\def\dots{\relax\ifmmode \ldots
          \else $\ldots$\fi}
\def\WHzsr{\ifmmode $W\,Hz\mo\,sr\mo$
           \else W\,Hz\mo\,sr\mo \fi}
\def\mKs{\ifmmode $\,mK\,s$^{-1/2} 
         \else \,mK\,s$^{-1/2}$ \fi}
\def\microns{\ifmmode \,\mu$m$
             \else \,$\mu$m\fi}
\def\micron{\microns}

%
\def\gsim{\lower.6ex\hbox{$\buildrel>\over\sim$}}
\def\lsim{\lower.6ex\hbox{$\buildrel<\over\sim$}}
\def\ra[#1 #2 #3.#4]{#1\sup{h}#2\sup{m}#3\sup{s}\llap.#4}
\def\dec[#1 #2 #3.#4]{#1\deg#2\arcm#3\arcs\llap.#4}
\def\deco[#1 #2 #3]{#1\deg#2\arcm#3\arcs}
%
\def\refindent{\hangindent=1em \hangafter=1 \noindent}
\def\ref #1;#2;#3;#4\par{\refindent #1,{\it #2},{\bf #3},#4.\par}
\def\ajref #1;#2;#3;#4\par{\refindent #1. #2 {\bf #3},#4.\par}
\def\vref #1\par{\refindent #1.\par}
\def\cref #1;#2;#3;#4;#5\par{\refindent #1, in{\it #2}, 
                             \hbox{ed.}#3 #4, \hbox{p.} #5.\par} 
\def\bref #1;#2;#3\par{\refindent #1, {\it #2} (#3).\par}
%
%
\def\tabl #1\par{\centerline{TABLE \number\tableno}
                 \vskip 7pt
                 \centerline{#1}\nointerlineskip\noindent}
\def\endtable{\tablewidth=\wd\tablebox 
    $$\hss\copy\tablebox\hss$$
    \vskip-\lastskip\vskip -2pt}
\def\tablenote#1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=\parindent \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotenoindent #1 #2\par{\begingroup \parindent=0.8em
    \abovedisplayshortskip=0pt\belowdisplayshortskip=0pt
    \noindent
    $$\hss\vbox{\hsize\tablewidth \hangindent=0pt \hangafter=1 \noindent
    \hbox to \parindent{\sup{\rm #1}\hss}\strut#2\strut\par}\hss$$
    \endgroup}
\def\tablenotes #1\par{
            \iftform \goodbreak\topinsert{
                 \centerline{NOTES TO TABLE \number\tableno}
                 \vskip .3cm\noindent
                 \eightpoint\input #1 }\endinsert
            \else \iftabsopen\relax
                  \else\immediate\openout\tabs=junk1\tabsopentrue\fi
                \vskip .5cm
                \centerline{NOTES TO TABLE \number\tableno} \vskip .5cm
                \immediate\write\tabs{\string\etable\space#1\string\par}
            \fi}
\def\doubleline{\vskip 3pt\hrule \vskip 1.5pt \hrule \vskip 5pt}
%
% macros for marginal stuff
%
\def\marginstuff#1{\setbox\marginbox=\vtop{
    \hsize=60pt\tolerance=10000\hbadness=10000
%    \hsize=70pt\tolerance=10000\hbadness=10000
    \parindent=0pt\eightpoint#1\par}\strut}
\def\setmarginal{\strut\vadjust{\kern-\strutdepth\kern-\ht\marginbox\vtop{%
    \moveleft 70pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%    \moveleft 80pt\hbox{\copy\marginbox}}\kern-\dp\marginbox\kern\strutdepth}}
%
% macro for absolute positioning on a page
%
\newdimen\offset 
\newdimen\unita \newdimen\unitb
\newdimen\mina  \newdimen\minb 
%
\unita=1.0cm \mina=0.0cm
\unitb=1.0in \minb=0.0in
%
%
\def\point #1 #2 #3;{\offset=#1\unitb\advance\offset by \minb%
    \rlap{\lower\offset\hbox{\hglue #2\unitb #3}}}%
%
% macros for memos
%
\font\ssq=cmssq8 at 7pt \font\ssbx=cmssbx10 at 12pt 
\setbox0=\hbox{\ssq ATENDEES \rm\quad}
\newdimen\atndwd \atndwd=\wd0
\def\file{}
\def\memo{\hsize=5.875in \hoffset=0.3125in
    \vsize=9in     \voffset=0in
    \elevenpoint
    \vglue -0.8in
    \line{\ssq\hfil INTEROFFICE MEMORANDUM\hfil \llap{\twelvepoint\bf\file}}
    \vskip 10pt
    \centerline{\hbox to 5.4in{\ssbx C A L I F O R N I A\hskip 12pt
                I N S T I T U T E\hskip 12pt O F\hskip 12pt 
                T E C H N O L O G Y}}
    \vskip 30pt}
\def\to#1{\line{\ssq TO \rm\quad #1\hfil\today}
          \vskip 12pt}
\def\from#1{\line{\ssq FROM \rm\quad C. R. Lawrence#1\hfil
                  \ssq EXTENSION \rm\quad 4976\quad\quad
                  \ssq MAIL CODE \rm\quad 105-24}
            \vskip 12pt}
\def\subject#1{\line{\ssq SUBJECT \rm\quad#1\hfil}
               \vskip 12pt}
\def\attendees#1{\hangindent=\atndwd \hangafter=1 \noindent
                \ssq ATENDEES \rm\quad#1
                \vskip 24pt}
\def\OVRO#1{\def\file{OVRO 5m \rlap{#1-87}}}

